AGVBench: A Reliability-Oriented Benchmark of Data Augmentation for Vein Recognition

Vein recognition is a secure biometric technology often constrained by limited annotated data and imaging variations. While data augmentation mitigates this, strategies designed for natural images may disrupt the fine-grained topology and textures essential for identity discrimination. We present AGVBench, which evaluates 30 representative augmentation strategies on five public palm- and finger-vein datasets with seven backbone architectures, covering classic CNNs, vision transformers, and vein-specific recognition models. Our results show that multi-image mixing methods (e.g., MixUp, PuzzleMix, StarMixup) generally provide the strongest recognition performance. However, they are often poorly calibrated and vulnerable to adversarial perturbations, revealing a clear inconsistency between clean accuracy and adversarial security. We also find that severe geometric transformations frequently degrade recognition, which is potentially due to feature misalignment or spatial cropping, and that augmentation effectiveness varies across palm and finger vein datasets. These findings prove that accuracy-centric evaluation is insufficient for biometric augmentation. AGVBench provides standardized protocols to support reproducible research and guide the design of reliable, secure, and robust vein recognition systems. Our codebase is available at https://github.com/Advance-VeinTech-Innovators/AGVBench.

==> Tabs/tab_aug_config.tex <==
\begin{table*}[htbp]
\centering
\caption{Configuration parameters and search spaces for various augmentation methods. The hyperparameter values represent the primary settings utilized in our empirical evaluation.}
\label{tab:augmentation_params}
\begin{tabularx}{\textwidth}{llX}
\toprule
\textbf{Method} & \textbf{Hyperparameter} & \textbf{Configuration / Search Space} \\
\midrule

% ==================== Single Image Augmentation ====================
\multicolumn{3}{c}{\textit{\textbf{Single Image Augmentation}}} \\
\midrule
Flip & Probability $p$ & $p = 0.5$ (Horizontal) \\
Rotate & Degree range $\theta$ & $\theta \in [-15^{\circ}, 15^{\circ}]$ \\
Translation & Shift ratio $(t_x, t_y)$ & $t_x, t_y \in [-0.1, 0.1]$ of image size \\
Blur & Kernel size $k$, Sigma $\sigma$ & $k \in \{3, 5, 7\}$, $\sigma \in [0.1, 2.0]$ \\
Noise & Variance $\sigma^2$ & Gaussian noise with $\sigma^2 \in [0.01, 0.05]$ \\
Cutout~\cite{devries2017cutout} & Number of holes $N$, Length $L$ & $N = 1$, $L \in [16, 32]$ pixels \\
GridMask~\cite{chen2020gridmask} & Block size $d$, Ratio $r$ & $d \in [24, 96]$, $r = 0.6$ \\
RandomErasing~\cite{zhong2020randome} & Prob. $p$, Area ratio $s_l, s_h$ & $p = 0.5$, $s_l = 0.02$, $s_h = 0.4$, Aspect ratio $r \in [0.3, 3.3]$ \\
RandomQuant~\cite{wu2023rq} & Quantization levels $q$ & $q \in \{4, 6, 8\}$ \\
AutoAugment~\cite{cubuk2019autoaugment} & Policy & Searched on ImageNet standard policy \\
RandAugment~\cite{cubuk2020randaugment} & Num ops $N$, Magnitude $M$ & $N = 2$, $M = 9$ (Magnitude range: 1 to 10) \\
KeepAugment~\cite{gong2021keepaugment} & Keep ratio $r$ & Saliency keep ratio $r = 0.6$ \\
TrivialAugment~\cite{muller2021trivialaugment}& Num ops $N$, Magnitude $M$ & $N = 1$, Magnitude uniformly sampled from $[1, 30]$ \\
TeachAugment~\cite{suzuki2022teachaugment} & Adversarial strategy & Online learned via teacher model guidance \\
SoftAugment~\cite{liu2023softaug} & Smoothing factor & Adaptive magnitude weighting \\
YOCO~\cite{han2022yoco}  & Split mode & Width/Height splitting with probability $0.5$ \\
\midrule

% ==================== Multi Image Augmentation ====================
\multicolumn{3}{c}{\textit{\textbf{Multi Image Augmentation}}} \\
\midrule
RICAP~\cite{takahashi2019ricap} & Beta distribution $\beta$ & $\beta = 0.3$ \\
MixUp~\cite{Zhang2018mixup} & Beta distribution $\alpha$ & $\alpha = 0.2$ (Weight $\lambda \sim \text{Beta}(\alpha, \alpha)$) \\
CutMix~\cite{Yun2019cutmix} & Beta distribution $\alpha$ & $\alpha = 1.0$ (Weight $\lambda \sim \text{Beta}(\alpha, \alpha)$) \\
FMix~\cite{Harris2020fmix} & Decay power $\delta$, Alpha $\alpha$ & $\delta = 3$, $\alpha = 1.0$ \\
GridMix~\cite{Baek2021gridmix} & Beta distribution $\alpha$ & $\alpha = 1.0$, grid size adapted to features \\
ResizeMix~\cite{Qin2020resizemix} & Beta distribution $\alpha$ & $\alpha = 1.0$, scaled patch insertion \\
AugMix~\cite{hendrycks2020augmix} & Mixture width $k$, Depth $d$ & $k = 3$, $d \in [1, 3]$, severity $= 3$, $\alpha = 1.0$ \\
SaliencyMix~\cite{Uddin2020saliencymix} & Beta distribution $\alpha$ & $\alpha = 1.0$, patch centered on saliency peak \\
PuzzleMix~\cite{Kim2020puzzle} & Alpha $\alpha$, Transport cost $\gamma$& $\alpha = 1.0$, $\gamma = 0.5$, Block size $= 4$ \\
GuidedMixup~\cite{kang2023guidedmixup} & Alpha $\alpha$, Attention norm & $\alpha = 1.0$, Guided by intermediate feature maps \\
StarMixup~\cite{jin2025starmixup} & Beta distribution $\alpha$ & $\alpha = 1.0$ \\
\midrule

% ==================== Label Enhancement ====================
\multicolumn{3}{c}{\textit{\textbf{Label Enhancement}}} \\
\midrule
LabelSmoothing~\cite{szegedy2016labelsmooth} & Smoothing factor $\epsilon$ & $\epsilon = 0.1$ \\
OnlineLabelSmooth~\cite{zhang2021onlinelabelsmooth}& Momentum $m$ & $m = 0.9$, updated dynamically per epoch \\
ConfidencePenalty~\cite{pereyra2017confidencepenalty}& Penalty weight $\lambda$ & Entropy regularization $\lambda = 0.1$ \\
DirichletLabelSmooth~\cite{cheng2021dirichletlabelsmoothLoss}& Dirichlet parameter $\alpha$ & $\alpha = 10.0$ over $K$ classes \\
Bootstrapping~\cite{reed2014bootstrapp} & Weight $\beta$, Mode & $\beta = 0.8$, Hard bootstrapping mode \\
\bottomrule
\end{tabularx}
\end{table*}
